ReTaSA: A Nonparametric Functional Estimation Approach for Addressing Continuous Target Shift

The presence of distribution shifts poses a significant challenge for deploying modern machine learning models in real-world applications. This work focuses on the target shift problem in a regression setting (Zhang et al., 2013; Nguyen et al., 2016). More specifically, the target variable y (also known as the response variable), which is continuous, has different marginal distributions in the training source and testing domain, while the conditional distribution of features x given y remains the same. While most literature focuses on classification tasks with finite target space, the regression problem has an infinite dimensional target space, which makes many of the existing methods inapplicable. In this work, we show that the continuous target shift problem can be addressed by estimating the importance weight function from an ill-posed integral equation. We propose a nonparametric regularized approach named ReTaSA to solve the ill-posed integral equation and provide theoretical justification for the estimated importance weight function. The effectiveness of the proposed method has been demonstrated with extensive numerical studies on synthetic and real-world datasets.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}


==> sections/numerical.tex <==
% !TEX root = ../iclr_supp.tex

% The performance of KDE requires a much larger sample size as the dimension of $\x$ increases.
% Inspired by \citep{lipton2018detecting}, we leverage the black-box models to address this issue.
% One of the methods to address this issue is to leverage the power of black-box models.
% We briefly discuss this approach and refer readers to \citep{lipton2018detecting} for more details.
% Lemma~1 in \citep{lipton2018detecting} suggests that we can replace $\x$ with $z=f(\x) \in \mathbb{R}$ as well as all the subsequent procedures.
% Thus, we avoid the curse of dimensionality and only apply the KDE on the scalar variable $z$.
% In the following, we will use the experiments to validate its performance.
% We can choose the mapping function $f(\cdot)$ as the estimated conditional mean function of a trained regression model on the source distribution: $z=\widehat{\mathbb{E}}_s(y|\x)$.
\subsubsection{Experiment with Multivariate Regression}
 
\textbf{Datasets.}
Our experiments are on the following two datasets: the synthetic multivariate regression dataset and the UCI 
Communities and Crime Dataset \citep{Dua2019}. In these two datasets, the features $\x$ are multivariate. Without loss of generality, we adopt the linear model as the linear regression model for both black-box mapping and prediction.
\begin{list}{\labelitemi}{\leftmargin=1em \itemindent=0em \itemsep=.2em}
    \item[1.] The synthetic multivariate regression dataset: The data are generated from the model $Y=\x\trans\boldsymbol{\beta}+ \epsilon$, where $\x,\boldsymbol{\beta}\in\mathbb{R}^5$ and $\epsilon \sim \text{Normal}(0,1)$.
The element values of $\x$ are generated from $\text{Normal}(0,1)$.  We set the regression coefficients with a randomly generated vector $\boldsymbol{\beta} = [1.132, 2.465, 7.776, 0, 0]^\top$. The data with top and bottom $5\%$ response values are filtered.
\item[2.] The UCI communities and crime dataset: The response variable $y$ is the logarithm of the total number of violent crimes per 100K population (\textit{ViolentCrimesPerPop}), and we predict it with the following features:  the number of vacant households (\textit{HousVacant}); the percent of housing occupied (\textit{PctHousOccup}); the percent of households owner occupied (\textit{PctHousOwnOcc}); the percent of vacant housing that is boarded up (\textit{PctVacantBoarded}); the percent of vacant housing that has been vacant more than six months (\textit{PctVacMore6Mos}); the percentage of people 16 and over, in the labor force, and unemployed (\textit{PctUnemployed}); the percentage of people 16 and over who are employed (\textit{PctEmploy}).
\end{list}
% For the Ames housing dataset, we treat the logarithm of the sale price (\textit{SalePrice}) as the response variable $y$.
%     The features are given below:
% \begin{list}{\labelitemi}{\leftmargin=1em \itemindent=0.2em \itemsep=.2em}
%         \item linear feet of street connected to property (\textit{Lot Frontage})
%         \item Original construction date (\textit{Year Built})
%         \item Type 1 finished square feet (\textit{BsmtFin SF 1})
%         \item Type 2 finished square feet (\textit{BsmtFin SF 2})
%         \item Unfinished square feet of basement area (\textit{Bsmt Unf SF})
%         \item Total square feet of basement area (\textit{Total Bsmt SF})
%         \item First floor square feet(\textit{1st Flr SF})
%         \item Second floor square feet (\textit{2nd Flr SF})
%         \item Low quality finished square feet (\textit{Low Qual Fin SF})
% \end{list}
    
\textbf{Continuous Target Shift Mechanism.}
We propose a bias sampling strategy to change the marginal distribution of the response $y$ to create a target shift.
Denote the empirical cumulative distribution function (cdf) of response $y$ in a raw dataset $\mathcal{D}$ as $\widehat{F}(y)$.
We first uniformly sample $n$ observations from the raw dataset and treat them as labeled source data.
For target data, we generate $m$ random numbers $\{u_i\}_{i=1}^{m}$ from some distribution with density $g(\cdot)$ on support $[0,1]$.
Then we pick the observations $\{(\x_i,y_i)\}$ from the raw dataset whose quantile of $y_i$ is $u_i$ (i.e., $\sup_{y}\{y|\widehat{F}(y)\leq u_i, y\in\mathcal{D}\}$), for $i=1,\dots,m$, as the target data.
Next, we show that under such a bias sampling strategy, the importance weight function is given by $\omega(y)=g\left\{\widehat{F}(y)\right\}$:
Letting the cdf of the raw data be $F(\cdot)$ and denote $U_1\sim\mathrm{uniform}(0,1)$
and $U_2\sim g(u)$.
Then random variable $F^{-1}(U_1)$ has the same distribution as the marignal distribution $p_s(y)$ while $F^{-1}(U_2)$ has the same distribution as $p_t(y)$.
Then distribution of $F^{-1}(U_1)$ is given by
$p_s(y)=g\left\{F(y)\right\}f(y)$,
where $f(y)$ is the corresponding pdf of $F(y)$.
Similarly, we have $p_t(y)=1\cdot f(y)$.
Thus, the importance weight function is
$\omega(y)=\frac{p_t(y)}{p_s(y)}=g\left\{F(y)\right\}$.
By replacing $F(\cdot)$ with the empirical $\widehat F(\cdot)$, we can obtain the ``true'' importance weight function.

One can see that if $g(\cdot)$ is uniform, the target and source data are from the same distribution (i.e., $\omega(y)=1$ for all $y$).
In our experiments, we use a truncated normal distribution $g(u)\sim\mathcal{TN}(\mu_t,\sigma_t^2,0,1)$.
%Then we obtain a sampled dataset as $\{\tilde{F}^{-1}(u_i)\}_{i=1}^{n}$, where $\tilde{F}^{-1}(u_i)$ is the largest value $y$ in the raw dataset of which the quantile is smaller than $u_i$.
%This sampling strategy results in the true importance weight as $\omega(y)=g\left\{F(y)\right\}$, where $g(u)$ is the density function of $u$. 
%We provide the detailed sampling algorithm and the true importance weight derivation in the supplementary.
%In our experiments, we use the uniform distribution $\mathcal{U}(0,1)$ and truncated normal distribution $\mathcal{TN}(\mu, \sigma^2, 0, 1)$ to generate $u$ for source and target data, respectively. 
Unless otherwise specified, we set $\mu_t=0.75$.
We use different values of $\sigma_t^2$ to adjust the shift, and a smaller value corresponds to a more severe shift.

% \textbf{Baseline Methods and Metric.}
% In our experiments, we consider three existing adaptation strategies as baseline methods:
% \begin{enumerate*}
%     \item[1).] Non-Adaptation, in which the source data trained model is directly applied for the prediction.
%     \item[2).] Oracle-Adaptation, of which the adaptation weight is the ground truth (i.e., $\omega(y_i) =\omega^*(y_i) =g_t\{\wh F_s(y)\}$).
%     \item[3).] KMM-Adaptation proposed in \cite{zhang2013domain}.
% \end{enumerate*}
% It is worth noting that Oracle Adaptation is infeasible in practice as the target shift mechanism (i.e., $g_t(\cdot)$) is unknown.

% Two metrics are adopted to evaluate the adaptation performance in our experiments: 1). Prediction MSE, which is the mean square error of the adapted response prediction (i.e., $\sum_{i=n+1}^{n+m}\|\hat{y}_i - y_i\|^2/m$); 2). Weight MSE, which is the mean square error of the estimated adaptation weights v.s. the ground-truth weights (i.e., $\sum_{i=n+1}^{n+m}\|\hat{\omega}(y_i) - \omega^*(y_i)\|^2/m$). Note that, for Non-Adaptation, we calculate the weight MSE by setting $\hat{\omega}(y_i) = 1$, for $i=n+1,\cdots,n+m$.
% It is worth noting that the target labels are masked from the adaptation procedure.

% \textbf{Hyperparameter Tuning.}
% Our proposed adaptation method involves two categories of hyperparameters: kernel bandwidths and a regularization parameter. For the first category, we use the kernel bandwidths to construct the matrices $\C_{\xi}$ and $\C_{\zeta}$. We adopt the median trick, as proposed in the works of \cite{zhang2013domain, garreau2017large}, to select the bandwidths. Specifically, for $\C_{\xi}$, we set the bandwidth $\nu_{\xi} = \frac{1}{2}\sqrt{H_{\xi,\tilde{n}}/2}$, where $H_{\xi,\tilde{n}}=\text{median}(\|\xi_{i}-\xi_{j}\|^2, 1\le i < j \le \tilde{n})$ is the median of the squared Euclidean distances between all pairs of samples in a subset of size $\tilde{n}$ drawn from the data. We choose $\tilde{n}$ as $\min \{n, 1000\}$ to reduce redundant computation. We follow a similar procedure to select the bandwidth for $\C_{\zeta}$.
% The second category of hyperparameters is the regularizer parameter $\alpha$. Choosing a large value of $\alpha$ leads to underfitting of the estimator $\rho$ as it is forced to be close to zero. Conversely, a small value of $\alpha$ leads to overfitting of $\rho$. Our experimental experience suggests that $\alpha$ can be determined by minimizing $C(\alpha) = \log(\|\C_{\zeta}\cdot(\C_{\xi}\rho_{\alpha} - \eta)\|^2/n) + \mathrm{Tr}(\C_{\zeta}(\alpha\I + \C_\xi\C_\zeta)^{-1})/2\log(n)$, where the two terms measure the fitting residual and the degree of freedom, respectively.
% We aim to strike a balance between the two terms to obtain an optimal value for $\alpha$.
% Additionally, we adopted the Gaussian kernel in all our experiments.

% \textbf{Comparison on Adaptation Methods.}
% In this part, we showcase the effectiveness of our proposed method in mitigating the negative impact of target shift.
% Linear regression is used as both the mapping and prediction models.
% We start with the setting of $\sigma=0.1$ and study the trade-off between adaptation performance and computation efficiency. 
% The experimental results are summarized in Table~\ref{tab.adaptation_comparison}. 
% Our results show that Oracle-Adaptation significantly outperforms Non-Adaptation in terms of prediction MSE. Specifically, on the synthetic, crime, and housing datasets, the prediction MSE was reduced by $12.9\%$, $74.6\%$, and $41.9\%$, respectively. These findings strongly suggest that efficient adaptation is crucial for optimal performance.
% Both KMM-Adaptation and our RECOLIA-Adaptation can mitigate the negative impact of target shift. 
% For example, KMM-Adaptation leads to a $9.6\%$ reduction in prediction MSE on the synthetic dataset, while our RECOLIA-Adaptation achieves an even more significant improvement of $11.0\%$ in prediction MSE.
% When considering the weight MSE metric, our RECOLIA-Adaptation consistently outperforms KMM-Adaptation across all three datasets. Specifically, our method reduces $59.0\%$, $5.8\%$, and $55.1\%$ on the synthetic, crime, and housing datasets, respectively.
% Furthermore, our RECOLIA-Adaptation yields significant improvements in computational efficiency, reducing the per-example computation time from at least $5$ seconds to just $0.2$ seconds compared to KMM-Adaptation.
% \begin{table}[ht]
%     \centering
%         \caption{The experimental results of adaptation performance and efficiency on the three datasets. The shift parameter $\sigma$ is fixed as 0.1. The numbers reported before and after $\pm$ symbolize the mean and standard deviation, respectively, after trimmed two-sided $5\%$ outliers.}
%     \label{tab.adaptation_comparison}
% \begin{tabular}{lc|ccc}
% \hline
% Dataset & Adaption &  Pred. MSE & Weight MSE &  Time (sec) \\
% \hline
%  \multirow{4}{*}{Synthetic} 
% &Oracle   &  $0.874_{\pm 0.056}$ &  - &  - \\
% &None     &  $1.004_{\pm 0.048}$ &  $1.866_{\pm 0.074}$ &  - \\
% &KMM      &  $0.907_{\pm 0.065}$ &  $0.593_{\pm 0.441}$ &  $8.984_{\pm 1.928}$ \\
% &RECOLIA    &  $0.894_{\pm 0.056}$ &  $0.243_{\pm 0.105}$ &  $0.216_{\pm 0.010}$ \\
% \hline
%  \multirow{4}{*}{Crime} 
% &Oracle   &  $0.116_{\pm 0.007}$ &  - &  - \\
% &None     &  $0.457_{\pm 0.043}$ &  $1.803_{\pm 0.086}$ &  - \\
% &KMM      &  $0.301_{\pm 0.035}$ &  $1.523_{\pm 0.094}$ &  $6.871_{\pm 1.343}$ \\
% &RECOLIA    &  $0.330_{\pm 0.035}$ &  $1.434_{\pm 0.076}$ &  $0.286_{\pm 0.023}$ \\
% \hline
%  \multirow{4}{*}{Housing} 
% &Oracle   &  $0.018_{\pm 0.004}$ &  - &  - \\
% &None     &  $0.031_{\pm 0.009}$ &  $1.858_{\pm 0.084}$ &  - \\
% &KMM      &  $0.028_{\pm 0.009}$ &  $1.608_{\pm 0.099}$ &  $5.192_{\pm 1.076}$ \\
% &RECOLIA    &  $0.026_{\pm 0.009}$ &  $0.722_{\pm 0.196}$ &  $0.209_{\pm 0.044}$ \\
% \hline
% \end{tabular}
% \end{table}

% Next, we tune the value of $\sigma$ to investigate the impact of the degree of target shift on the adaptation performance, and the experimental results are shown in Figure~\ref{fig.MSE_over_Sigma}. As the degree of shift increases, the prediction MSEs of the adapted methods are consistently smaller than those from Non-Adaptation. Furthermore, both KMM-Adaptation and our RECOLIA-Adaptation demonstrate similar performance under different degrees of shift. Taking computational efficiency into consideration, we can conclude that our RECOLIA-Adaptation provides an effective and efficient approach for mitigating the negative impact of target shift.

% \begin{figure}[ht!]
% \centering
% \begin{tabular}{@{}ccc@{}}
% % \includegraphics[width=0.32\linewidth]{figures/synthetic_weight_mse_over_sigma.pdf} &
% % \includegraphics[width=0.32\linewidth]{figures/crime_weight_mse_over_sigma.pdf} & 
% % \includegraphics[width=0.32\linewidth]{figures/ames_weight_mse_over_sigma.pdf}\\
% \includegraphics[width=0.32\linewidth]{figures/synthetic_prediction_mse_over_sigma.pdf} &
% \includegraphics[width=0.31\linewidth]{figures/crime_prediction_mse_over_sigma.pdf} &
% \includegraphics[width=0.31\linewidth]{figures/ames_prediction_mse_over_sigma.pdf}\\
% (a) Synthetic Dataset & (b) Crime Dataset & (c) Housing Dataset\\
% \end{tabular}
% \caption{Prediction v.s. the degree of shift. We control the target shift by adjusting $\sigma$. The solid curves represent the median, and the shadow regions are $95\%$ CI error band.}\label{fig.MSE_over_Sigma}
% \end{figure}


% \textbf{Impact of Black-box Model for feature dimension reduction.}
% In this experiment, we aim to assess the impact of black-box model choice on adaptation performance.
% We have set the target shift setting to a fixed value of $\sigma = 0.1$, and we will be using the linear regression model for prediction.
% To evaluate the impact of black-box model choice, we will compare the performance of different black-box models, including decision tree regression, kernel ridge regression, linear regression, multi-layer perceptron, and random forest regression. 
% All these models have been implemented using the "scikit-learn" Python package. 
% The multi-layer perceptron model has been set to run with a maximum iteration of 500, while the other mapping models have been left at their default settings.

% The experimental results are presented in Table~\ref{tab.model_misspecification}. Our analysis reveals that the random forest model has the lowest weight MSEs across all three datasets, while the overall prediction MSE is roughly similar across different mapping models. Additionally, we observe that smaller-weight MSEs generally correspond to smaller prediction MSEs.

% \begin{table}[ht!]
%     \centering
%      \caption{The adaptation performance on the three datasets with different mapping models. The shift parameter $\sigma$ is fixed as 0.1. The numbers reported before and after $\pm$ symbolize the mean and standard deviation, respectively, after trimmed two-sided $5\%$ outliers.}
%         \label{tab.model_misspecification}
% \begin{tabular}{lc|cc}
% \hline
% Dataset & Model &  Pred. MSE & Weight MSE  \\
% \hline
%  \multirow{5}{*}{Synthetic} 
% &Decision Tree           &  $0.914_{\pm 0.053}$ &  $0.127_{\pm 0.047}$ \\
% &Kernel Ridge Regression           &  $0.894_{\pm 0.056}$ &  $0.243_{\pm 0.105}$ \\
% &Linear Regression                &  $0.894_{\pm 0.056}$ &  $0.243_{\pm 0.105}$ \\
% &Multi-layer Perceptron &  $0.890_{\pm 0.057}$ &  $0.189_{\pm 0.080}$ \\
% &Random Forest          &  $0.896_{\pm 0.054}$ &  $0.085_{\pm 0.042}$ \\
% \hline
%  \multirow{5}{*}{Crime} 
% &Decision Tree           &  $0.359_{\pm 0.040}$ &  $1.497_{\pm 0.084}$ \\
% &Kernel Ridge Regression           &  $0.378_{\pm 0.038}$ &  $1.585_{\pm 0.082}$ \\
% &Linear Regression                &  $0.330_{\pm 0.035}$ &  $1.434_{\pm 0.076}$ \\
% &Multi-layer Perceptron  &  $0.423_{\pm 0.048}$ &  $1.711_{\pm 0.110}$ \\
% &Random Forest           &  $0.297_{\pm 0.036}$ &  $1.311_{\pm 0.095}$ \\
% \hline
%  \multirow{5}{*}{Housing} 
% &Decision Tree           &  $0.027_{\pm 0.009}$ &  $0.946_{\pm 0.163}$ \\
% &Kernel Ridge Regression         &  $0.026_{\pm 0.009}$ &  $0.718_{\pm 0.190}$ \\
% &Linear Regression                 &  $0.026_{\pm 0.009}$ &  $0.722_{\pm 0.196}$ \\
% &Multi-layer Perceptron  &  $0.030_{\pm 0.009}$ &  $1.831_{\pm 0.094}$ \\
% &Random Forest           &  $0.025_{\pm 0.009}$ &  $0.612_{\pm 0.174}$ \\
% \hline
% \end{tabular}
% \end{table}

% \textbf{Sensitivity Analysis of Regularization.}
% Our final experiment aims to conduct a sensitivity analysis of the RECOLIA-Adaptation method with respect to the regularization parameter $\alpha$. It is worth noting that a larger value of $\alpha$ will push the estimated adaptation weight towards $1$, while a smaller $\alpha$ will result in a larger estimation variation. As in our previous experiments, we fix $\sigma$ to $0.1$ and use linear regression models for both mapping and prediction.

% Our experimental results are presented in Figure~\ref{fig.MSE_over_alpha}. The red dashed line in the figure represents the Oracle Adaptation, which uses the ground-truth weights $\omega^*(y)$ and has zero-weight MSEs. The black line denotes the weight MSEs for Non-Adaptation, which is calculated as $\sum_{i=n+1}^{n+m}|1 - \omega^*(y_i)|^2/m$. We range $\alpha$ from 0.01 to 10 for our RECOLIA-Adaptation and show the corresponding weight MSEs using the blue curve. Additionally, we mark the results obtained using the tuned $\alpha$ with a star marker. Our analysis reveals that both very small and very large values of $\alpha$ lead to poor adaptation estimation, as can be observed in Figure~\ref{fig.MSE_over_alpha}(a) and (c). 
% While our proposed tuning method can identify a relatively reasonable value for $\alpha$, it is worth noting that the properties of the data can heavily influence the choice of $\alpha$.
% Since finding the best $\alpha$ in all scenarios is a highly non-trivial task, we leave it for future investigation.

\begin{table}[t!]
    \centering
        \caption{The experimental results of adaptation weight estimation and improved prediction performance on the synthetic multivariate regression datasets. The numbers reported before and after $\pm$ symbolize the mean and standard deviation, respectively. The bold values are the results with the best performance, while Oracle-Adaptation is excluded due to being practically feasible. }
    \label{tab:synthetic_result}
    \begin{tabular}{ll|ccc|c:cc}
\hline
 \multicolumn{2}{l|}{Setting}  & \multicolumn{3}{c|}{Weight MSE} & \multicolumn{3}{c}{$\Delta$Pred. MSE (\%)} \\
 \hline
$n$ & Shift & None & KMM & Ours & Oracle & KMM & Ours \\
\hline
\multirow[c]{3}{*}{200}  &Mild & $\mathbf{0.01_{\pm 0.00}}$ & $0.10_{\pm 0.06}$ & ${0.02_{\pm 0.01}}$ & $0.07_{\pm 0.43}$ & $0.07_{\pm 1.31}$ & $\mathbf{0.16_{\pm 0.60}}$ \\
 &Moderate & $0.07_{\pm 0.00}$ & $0.08_{\pm 0.05}$ & $\mathbf{0.02_{\pm 0.01}}$ & $0.25_{\pm 1.07}$ & $-0.01_{\pm 1.46}$ & $\mathbf{0.24_{\pm 0.89}}$ \\
 &Intense & $0.31_{\pm 0.01}$ & $0.08_{\pm 0.05}$ & $\mathbf{0.03_{\pm 0.01}}$ & $0.61_{\pm 1.94}$ & $0.68_{\pm 1.84}$ & $\mathbf{0.73_{\pm 1.28}}$ \\
\cline{1-8}
\multirow[c]{3}{*}{500} &Mild & $\mathbf{0.01_{\pm 0.00}}$ & $0.05_{\pm 0.02}$ & $0.01_{\pm 0.01}$ & $-0.02_{\pm 0.21}$ & $-0.12_{\pm 0.61}$ & $-0.03_{\pm 0.29}$ \\
 &Moderate & $0.07_{\pm 0.00}$ & $0.05_{\pm 0.03}$ & $\mathbf{0.01_{\pm 0.01}}$ & $0.04_{\pm 0.62}$ & $-0.11_{\pm 0.81}$ & $\mathbf{0.02_{\pm 0.54}}$ \\
 & 
Intense & $0.32_{\pm 0.01}$ & $0.04_{\pm 0.03}$ & $\mathbf{0.02_{\pm 0.01}}$ & $1.01_{\pm 1.17}$ & $0.86_{\pm 1.17}$ & $\mathbf{0.95_{\pm 0.88}}$ \\
\cline{1-8}
\multirow[c]{3}{*}{1000} &Mild & $\mathbf{0.01_{\pm 0.00}}$ & $0.02_{\pm 0.01}$ & $0.01_{\pm 0.01}$ & $0.03_{\pm 0.11}$ & $-0.06_{\pm 0.21}$ & $-0.02_{\pm 0.12}$ \\
 &Moderate & $0.08_{\pm 0.00}$ & $0.02_{\pm 0.01}$ & $\mathbf{0.01_{\pm 0.01}}$ & $0.14_{\pm 0.46}$ & $0.08_{\pm 0.52}$ & $\mathbf{0.11_{\pm 0.41}}$ \\
 &Intense & $0.32_{\pm 0.01}$ & $0.03_{\pm 0.02}$ & $\mathbf{0.02_{\pm 0.01}}$ & $1.21_{\pm 0.75}$ & $\mathbf{1.17_{\pm 0.74}}$ & $1.14_{\pm 0.57}$ \\
\hline
\end{tabular}
\end{table}


\begin{table}[t!]
    \centering
        \caption{The experimental results of adaptation weight estimation and improved prediction performance on the UCI communities and crime datasets. The numbers reported before and after $\pm$ symbolize the mean and standard deviation, respectively. The bold values are the results with the best performance, while Oracle-Adaptation is excluded due to being practically feasible.}
    \label{tab:crime_result}
    \begin{tabular}{ll|ccc|c:cc}
\hline
 \multicolumn{2}{l|}{Setting}  & \multicolumn{3}{c|}{Weight MSE} & \multicolumn{3}{c}{$\Delta$Pred. MSE (\%)} \\
 \hline
$n$ & Shift & None & KMM & Ours & Oracle & KMM & Ours \\
\hline
\multirow[c]{3}{*}{200} & Mild & $\mathbf{0.01_{\pm 0.00}}$ & $1.34_{\pm 0.43}$ & $0.01_{\pm 0.01}$ & $1.44_{\pm 1.87}$ & $-24.35_{\pm 29.51}$ & $\mathbf{0.65_{\pm 2.15}}$ \\
 & Moderate & $0.08_{\pm 0.01}$ & $1.24_{\pm 0.47}$ & $\mathbf{0.04_{\pm 0.03}}$ & $8.84_{\pm 5.10}$ & $-13.32_{\pm 33.03}$ & $\mathbf{4.93_{\pm 3.76}}$ \\
 & 
Intense & $0.33_{\pm 0.02}$ & $1.24_{\pm 0.61}$ & $\mathbf{0.14_{\pm 0.04}}$ & $31.06_{\pm 9.16}$ & $13.72_{\pm 34.91}$ & $\mathbf{18.41_{\pm 5.20}}$ \\
\cline{1-8}
\multirow[c]{3}{*}{500}  & Mild & $\mathbf{0.01_{\pm 0.00}}$ & $1.28_{\pm 0.49}$ & $0.01_{\pm 0.01}$ & $0.67_{\pm 1.45}$ & $-8.64_{\pm 10.25}$ & $\mathbf{0.55_{\pm 0.90}}$ \\
 & Moderate & $0.08_{\pm 0.00}$ & $1.23_{\pm 0.54}$ & $\mathbf{0.04_{\pm 0.02}}$ & $7.05_{\pm 4.17}$ & $-2.35_{\pm 14.38}$ & $\mathbf{4.47_{\pm 2.54}}$ \\
 & Intense & $0.33_{\pm 0.01}$ & $1.11_{\pm 0.59}$ & $\mathbf{0.13_{\pm 0.03}}$ & $29.11_{\pm 5.80}$ & $17.22_{\pm 14.28}$ & $\mathbf{19.83_{\pm 3.69}}$ \\
\cline{1-8}
\multirow[c]{3}{*}{1000}  & Mild & $\mathbf{0.01_{\pm 0.00}}$ & $0.92_{\pm 0.31}$ & $0.01_{\pm 0.01}$ & $0.68_{\pm 0.71}$ & $-4.29_{\pm 5.23}$ & $\mathbf{0.42_{\pm 0.64}}$ \\
 & Moderate & $0.08_{\pm 0.00}$ & $0.88_{\pm 0.31}$ & $\mathbf{0.03_{\pm 0.01}}$ & $6.45_{\pm 2.28}$ & $-0.72_{\pm 7.03}$ & $\mathbf{4.52_{\pm 1.54}}$ \\
 & Intense & $0.33_{\pm 0.01}$ & $0.77_{\pm 0.30}$ & $\mathbf{0.10_{\pm 0.02}}$ & $28.51_{\pm 3.57}$ & $\mathbf{24.24_{\pm 6.15}}$ & $22.36_{\pm 2.41}$ \\
\hline
\end{tabular}
\end{table}

\textbf{Performance Comparison}. In this part, we showcase the effectiveness of our proposed method in mitigating the negative impact of target shift. Without a loss of generality, the linear regression model is used for the feature dimension reduction and response prediction.
We aim to study the methods' performances under different sample sizes and shift settings. In our study, the sample size ranges from $\{200, 500, 1000\}$ and $\sigma_t^2$ is from $\{0.3, 0.5, 0.9\}$. Note that as $\sigma_t^2$ increases, the truncated normal distribution becomes flat, and thus, the shift becomes mild. Thus, we represent the $\sigma_t^2$ settings with three shift levels, \{Mild: $\sigma_t^2=0.9$,  Moderate: $\sigma_t^2=0.5$, Intense: $\sigma_t^2=0.3$\}. We reproduce the experiments with 20 trials for each setting.

The experimental results are summarized in Table~\ref{tab:synthetic_result}-\ref{tab:crime_result}.
First, in terms of weight estimation, our method consistently outperforms KMM-Adaptation across all settings. When applied to the crime dataset, KMM-Adaptation experiences significant estimation errors, performing much worse than Non-Adaptation. In contrast, our method maintains low-weight MSE.
Secondly, regarding response prediction, our method consistently surpasses KMM-Adaptation, closely approaching the performance of Oracle-Adaptation across a wide range of settings. Even though KMM-Adaptation exhibits slightly better in $\Delta$Prediction MSE than our method with $n=1000$ and intense shift, it's important to highlight that the corresponding standard deviation of KMM-Adaptation is significantly higher than that of our method. Consequently, we believe that our method consistently outperforms KMM-Adaptation.


